On the Robustness of Dataset Inference

Machine learning (ML) models are costly to train as they can require a significant amount of data, computational resources and technical expertise. Thus, they constitute valuable intellectual property that needs protection from adversaries wanting to steal them. Ownership verification techniques allow the victims of model stealing attacks to demonstrate that a suspect model was in fact stolen from theirs. Although a number of ownership verification techniques based on watermarking or fingerprinting have been proposed, most of them fall short either in terms of security guarantees (well-equipped adversaries can evade verification) or computational cost. A fingerprinting technique, Dataset Inference (DI), has been shown to offer better robustness and efficiency than prior methods. The authors of DI provided a correctness proof for linear (suspect) models. However, in a subspace of the same setting, we prove that DI suffers from high false positives (FPs) -- it can incorrectly identify an independent model trained with non-overlapping data from the same distribution as stolen. We further prove that DI also triggers FPs in realistic, non-linear suspect models. We then confirm empirically that DI in the black-box setting leads to FPs, with high confidence. Second, we show that DI also suffers from false negatives (FNs) -- an adversary can fool DI (at the cost of incurring some accuracy loss) by regularising a stolen model's decision boundaries using adversarial training, thereby leading to an FN. To this end, we demonstrate that black-box DI fails to identify a model adversarially trained from a stolen dataset -- the setting where DI is the hardest to evade. Finally, we discuss the implications of our findings, the viability of fingerprinting-based ownership verification in general, and suggest directions for future work.

==> explanations.tex <==
\section{Some explanation}
% First, recall that the victim has access to its own private training set of size $m$. For the purposes of this proof, we call it $S_V$. 
% As the victim has complete information of the data distribution, it can randomly sample another dataset $S_0 \sim D$.

% The victim considers that the potential adversary’s model was stolen if the mean ‘prediction margin’ for the points in $S_V$ is greater than $S_0$ by some threshold parameter $\lambda$. Let $\Psi_V (f, S; D)$ be V’s decision function to resolve ownership claims.

% Let $t_V$ represent the mean of the ‘prediction margin’ of k verify points in $S_V$ for a classifier
% f. Similarly, let $t_0$ represent the mean of the ‘prediction margin’ of k verify points in $S_0$ for the classifier
% f.

\begin{enumerate}
    \item $S_v$: training set of size $m$ for victim
    \item $S_0$: another dataset following the same distribution $D$
    \item $\Psi_V (f, S; D)$: DI decision function, 1 for stolen model
    \item $t_v$: the mean of prediction margin of all points in $S_v$
    \item $t_0$: the mean of prediction margin of all points in $S_0$
\end{enumerate}


DI claims that a model is stolen if:
$P [\Psi_V (f, S; D) = 1] = P [(t_V - t_0) > \lambda]$.

\begin{equation*}
    \begin{aligned}
         t_v =& \frac{1}{m}\sum_j^m[\sum_i^{i\neq j}y^{(i)}x_2^{(i)}x_2^{(j)}+y^{(j)}x_2^{(j)}x_2^{j}],\\
         t_0 =& \frac{1}{m}\sum_j^m[\sum_i y^{(i)}x_2^{(i)}x_2^{(j)}],
    \end{aligned}
\end{equation*}

where $t_v\sim N(D\sigma^2,D\sigma^4)$, $t_0\sim N(0,D\sigma^4)$.

When selecting k points for verify,
\begin{equation*}
    \begin{aligned}
         t_v =& \frac{1}{k}\sum_j^k[\sum_i^{m,i\neq j}y^{(i)}x_2^{(i)}x_2^{(j)}+y^{(j)}x_2^{(j)}x_2^{j}],\\
         t_0 =& \frac{1}{k}\sum_j^k[\sum_i^m y^{(i)}x_2^{(i)}x_2^{(j)}],
    \end{aligned}
\end{equation*}

\textbf{For the true positive}, $t_v=t_0$, $t_V-t_0 \sim N(0,\frac{2m}{k}D\sigma^4)$,
\begin{equation*}
    \begin{aligned}
         P [t_V - t_0 > \lambda] = P[Z\sigma_t+\mu_t>\lambda]=1-\Phi(-\frac{\sqrt{kD}}{2\sqrt{2m}}).
    \end{aligned}
\end{equation*}

It means when k is small compared to m, $P\to 0.5$

\textbf{For the false positive}, $t_v=t_0$, $t_V-t_0 \sim N(0,\frac{2m}{k}D\sigma^4)$,
\begin{equation*}
    \begin{aligned}
         P [t_V - t_0 > \lambda] = P[Z\sigma_t>\lambda]=P[Z>\frac{\lambda}{\sigma_t}]=P[Z>\frac{\sqrt{k}\lambda}{\sqrt{2Dm}\sigma^2}]=1-\Phi(\frac{\sqrt{k}\lambda}{\sqrt{2Dm}\sigma^2}).
    \end{aligned}
\end{equation*}

When $\lambda$ is a constant, when $D\to \infty$, $P[\hat{t}>\lambda] \to 0.5$.

\textbf{For the overlapping dataset}, if there are p dependent points, $t_0=t_v$, $t_V-t_0 \sim N(\frac{k-p}{k}D\sigma^2,\frac{2m}{k}D\sigma^4)$, and let $\lambda=\frac{\mu_t}{2}$
\begin{equation*}
    \begin{aligned}
         P [|t_V - t_0| > \lambda] = P[Z\sigma_t+\mu_t>\lambda]=1-\Phi(-\frac{(k-p)\sqrt{D}}{2\sqrt{2mk}}).
    \end{aligned}
\end{equation*}
It means that when $p \to k$, $P\to 0.5$.

\textbf{For the MI}, $t_v,t_0$ means any sample in the dataset $S_v,S_0$,
\begin{equation*}
    \begin{aligned}
         P [|t_V - t_0| > \lambda] = P[Z\sigma_t+\mu_t>\lambda]=1-\Phi(-\frac{\sqrt{D}}{2\sqrt{2m}}).
    \end{aligned}
\end{equation*}
D and m can both be very large.
If we use MI for the whole dataset...

\paragraph{Hypothesis Tests.} We query models with equal number of samples from public and private
datasets, create embeddings and calculate confidence score vectors $c$ and $c_V$ , respectively. We
form a two sample T-test on the distribution of $c$ and $c_V$ and calculate the p-value for the one-sided
hypothesis $H0 : \mu < \mu_V$ against $H_a : \mu > \mu_V$ . From L(x, y), it follows that $g_V$ learns to minimize
$g_V (x)$ when $x \in S_V$ maximizes it otherwise. Therefore, a vector that contains samples from
$S_V$ produces lower confidence scores, and decreases the test’s p-value. If the p-value is below a
predefined significance level $\alpha$, $H_0$ is rejected, and the model under test is marked as ‘stolen’.


\textbf{For true positive}, $\mu_V$ should be small and $\mu$ should be large.


\textbf{For false positive}, 
$\mu_V$ should be large and $\mu$ should be large. Then $\Delta \mu = \mu-\mu_V$... 

\textbf{Another $g$ for public dataset: we use $g_v$ for $S_v$, and $g_0$ for $S_0$.}

Assuming that the victim model is trained on private dataset $S_v$, then the distance is measured by two-layer linear model $g_v$. The loss function is $L_v(f, x, y, S_v) = g_v$, the output of function $g_v$ is the confidence about a data point's membership in dataset $S_v$.

Assuming that the attack model is trained on dataset $S_0$, 
Then the problem of training $g$ is two-fold.
\begin{enumerate}
    \item If the dataset $S_0$ is public.
    \item If the dataset $S_0$ is private.
\end{enumerate}
 
 If $S_0$ is public, a two-layer linear model $g$ can be trained on $S_0$ directly with loss function $L_v(f_v, x, y, S_0) = g$. The output of function $g$ is the confidence about if data point $x$ belongs to $S_0$. 
 
 If $S_0$ is private, similar to DI which reveal $m$ samples to their verification, the adversary are required to reveal $m$ samples to prove their innocence, which denoted as $S_0^m$. We use $S_0^m$ to train model $g$ with loss function $L_v(f, x, y, S_0) = g$. 
 
 Compared the public case, the $g$ might be larger because it is trained on a subset of $S_0$. 
 We could extend $S_0^m$ with data points randomly sampled from distribution $D$, until the size of $S_0^m$ equals the size of $S_0$. And we train a new model $\hat{f}$ on the extended dataset $\hat{S}_0$. Then we use $g$ to estimate this new model $\hat{f}$ and get the baseline $\hat{\mu}$.
 
 Also, for the public case, we train a new model on $S_0$ and get the base line $\hat{\mu}$
 Finally, we could compare the distance $\mu-\mu_v$ and base line $\hat{\mu}-\mu_v$. 

% For the adversary, $t_V-t_0 \sim N(D\sigma^2,\frac{2m}{k}D\sigma^4)$. For a honest adversary, $\hat{t}=t_V-t_0 \sim N(0,\frac{2m}{k}D\sigma^4)$.
% False positive: $P [\Psi_V (f, S; D) = 1] = P [\hat{t}=(t_V - t_0) > \lambda]$. Let $Z\sim N(0,1)$,
% \begin{equation*}
%     \begin{aligned}
%          P [\hat{t}=(t_V - t_0) > \lambda] = P[Z\sigma_t>\lambda]=P[Z>\frac{\lambda}{\sigma_t}]=P[Z>\frac{\sqrt{k}\lambda}{\sqrt{2Dm}\sigma^2}]=1-\Phi(\frac{\sqrt{k}\lambda}{\sqrt{2Dm}\sigma^2})
%     \end{aligned}
% \end{equation*}
% When $\lambda$ is a constant, when $D\to \infty$, $P[\hat{t}>\lambda] \to 0.5$.
% \section{Some examples to get started}


==> makefile <==
all :
	{ \
		pdflatex -synctex=1 -interaction=nonstopmode --shell-escape main ;\
		bibtex main;\
		pdflatex -synctex=1 -interaction=nonstopmode --shell-escape main ;\
		pdflatex -synctex=1 -interaction=nonstopmode --shell-escape main ;\
	}

sweep :
	rm -f *.log *.aux *.out *.synctex.gz *.blg *.brf *.fls *.fdb_latexmk *.xmpi *.toc *.xmpdata

cleanpdf:
	rm -f *.pdf

clean : sweep cleanpdf

